Planets around stars in young nearby associations *** radial Velocity searches: a feasibility study, and first results

Stars in young nearby associations are the only targets allowing giant planet searches at all separations in the near future, by coupling indirect techniques such as radial velocity and deep imaging. These stars are first priorities targets for the forthcoming planets imagers on 10-m class telescopes. Young stars rotate more rapidly and are more active than their older counterparts. Both effects can limit the capability to detect planets using RV. We wish to explore the planet detection capabilities of a representative sample of stars in close and young associations with radial velocity data and explore the complementarity between this technique and direct imaging. We observed 26 such targets with spectral types from A to K and ages from

==> biblio.tex <==
\begin{thebibliography}{}
	\bibitem[Aigrain et al. 2012]{aigrain12} Aigrain, S., Pont, F., Zucker, S., 2012, MNRAS, 419, 3147
	\bibitem[Bailey et al. 2012]{bailey12} Bailey, J.I. III, White, R. J., Blake, C. H., et al, 2012 ApJ, 749, 16
	\bibitem[Beuzit et al. 2008]{beuzit08} Beuzit, J.L., Feldt, M., Dohlen, K., et al, 2008, SPIE, 7014, 41
	\bibitem[Buenzli et al. 2010]{buenzli10}     Buenzli, E., Thalmann, C., Vigan, A., et al, 2010,  A\&A, 524, L1
	\bibitem[Boisse et al. 2009]{boisse09} Boisse, I., Moutou, C., Vidal-Madjar, A., et al, 2009, A\&A, 459, 959
	\bibitem[Boisse et al. 2011]{boisse11} Boisse, I., Bouchy, F., hebrard, G., et al, 2009, A\&A, 528, 4
	\bibitem[Chelli]{chelli00}     Chelli, A., 2000, A\&A 358, L59
	\bibitem[Chiang et al.\ 2009]{chiang09} Chiang, E., Kite, E., Kalas, P. et al, 2009, ApJ, 693, 734
  	\bibitem[Desort et al. \ 2007]{desort07}     Desort, M., Lagrange, A.-M., Galland, F., et al., 2007, A\&A 473, 983
% \bibitem[Desort et al. 2008]       {desort08}     Desort, M., Lagrange, A.-M., Galland, F., et al., 2008, A\&A 491, 883
%  \bibitem[Desort et al. 2009]       {desort09}     Desort, M., Lagrange, A.-M., Galland, F., et al., 2009, A\&A, 506, 1469
\bibitem[Desidera et al. 2011]{desidera11} DesideraS., Covino E., Messina S., et al, 2011, A\&A, 529, 54
	\bibitem[Dumusque et al. 2011]{dumusque11} Dumusque, X., Lovis, C., Ségransan, D., et al, 2011, A\&A, 535, A55
\bibitem[Duncan et al. 1991] {duncan91} Duncan, D. K., Vaughan, A. H., Wilson, O. C.,  et al, 1991, ApJS, 76, 833
	\bibitem[Frankowski et al. 2007]{frankowski07} Frankowski, A., Jancart, S., et al, 2007, A\&A, 464, 377
	\bibitem[Galland et al. 2005]{galland05a}   Galland, F., Lagrange, A.-M., Udry, S., et al., 2005, A\&A 443, 337
%\bibitem[Galland et al. 2005b]      {galland05b}   Galland, F., Lagrange, A.-M., Udry, S., et al., 2005b, A\&A 444, L21
%\bibitem[Galland et al. 2006]      {galland06}   Galland, F., Lagrange, A.-M., Udry, S., et al., 2006b, A\&A 452, 709
	\bibitem[Garcia-Alvarez et al. 2011]{alvarez11} Garcia-Alvarez, D., Lanza, A. F., Messina, S., et al, 2011, A\&A, 533, 30
	\bibitem[Hines et al. 2007] {hines07}Hines, D. C., Schneider, G., Hollenbach, D., et al, 2007, ApJ, 671, L167
	\bibitem[Isaacson and Fisher et 2010]{isaacson10} Isaacson, H., and Fischer, D., 2010, ApJ, 725, 875
	\bibitem[Kalas et al.\ 2005]{kalas05} Kalas, P., Graham, J. R., Clampin, M., 2005, Nature, 435, 1067
	\bibitem[Kalas et al.\ 2008]{kalas08} Kalas, P., Graham, J. R., Chiang, E., et al,  2008, Science, 322, 1345
	\bibitem[Kalas et al. 2011]{kalas11} Kalas, Paul, Fitzgerald, M. P., Papadopoulos, P. P., Graham, J. R., Bulletin of the American Astronomical Society, 42, 587
	\bibitem[Lagrange et al.\ 2009]{lagrange09b} Lagrange, A.M, Desort, M., Galland, F., et al, 2009b, A$\&$A, 495, 335
	\bibitem[Lagrange et al.\ 2009a]{lagrange09a} Lagrange, A.M., Gratadour, D., Chauvin, G., et al, 2009b,  A\&A, 493, L21
%\bibitem[Lagrange et al.\ 2009b] {lagrange09b} Lagrange, A.M., Kasper, M., Boccaletti, A. et al, A\&A, 506, L927
	\bibitem[Lagrange et al.\ 2010]{lagrange10} Lagrange, A.M., Bonnefoy, M., Chauvin, G., et al, 2010, Science, 329, L57
	\bibitem[Lagrange et al.\ 2012]{lagrange12} Lagrange, A.M., De Bondt, K., Meunier, N., et al, 2012, A\&A, 542, 18
	\bibitem[Lanza et al.\ 2011]{lanza11} Lanza, A. F., Boisse, I., Bouchy, F., et al,  2011, A\&A, 533, 44
	\bibitem[Lebreton et al.\ 2012]{lebreton12}	Lebreton, J., Augereau, J.-C., Thi, W.-F., et al, 2012, A\&A, 539, 17
	\bibitem[Lockwood et al.\ 2007]{lockwood07} Lockwood, G. W., Skiff, B. A., Henry, Gregory W., et al, 2007, ApJS, 171, 260
	\bibitem[Mayor et al. 2011]{mayor11} Mayor, M., Marmier, M., Lovis, C., et al, 2011, arXiv:1109.2497
	\bibitem[Marois et al.\ 2008] {marois08} Marois, C., MacIntosh, B., Barman, T., Zuckerman, B., Inseok, S., Patience, J., Lafreniere, D., Doyon, R. 2008, Science, 322, 1348
	\bibitem[Macintosh et al. \ 2008]{macintosh08}Macintosh, B. A., Graham, J. R., Palmer, D. W., et al,  2008, SPIE, 7015, 31
	\bibitem[Marois et al.\ 2010]{marois10} Marois, C., Zuckerman, B., Konopacky, Q. M., Macintosh, B., Barman, Travis, 2010, Nature, 468, 1080
\bibitem[Marois et al. 2008]{marois08} Marois, C., et al, 2008 GPI
	\bibitem[Meunier et al.\ 2012]{meunier12} Meunier, N., Lagrange, A.-M., De Bondt, K., 2012, A\&A, accepted, 2012arXiv1207.4329
	\bibitem[Meunier and Lagrange \ 2012b]{meunier12b} Meunier, N., Lagrange, A.-M., 2012, A\&A, submitted
	\bibitem[Moor et al.\ 2006]{moor06} Moor, A, Abraham, P., Derekas, A. et al, 2006, ApJ, 644, 525
	\bibitem[Mugrauer et al.\ 2010]{mugrauer10} Mugrauer M., Vogt N., Neuhaueser R. and Schmidt, T.O.B. , 2010, A\&A, 523, L1
	\bibitem[Patience et al. 2011]{patience11}    Patience, J., Bulger, J., King, R.R., et al, 2011, ApJ, 531, L17 
	\bibitem[Rhee et al. 2007]{rhee07} Rhee, J.H., Song I., Zuckerman B., and McElwain, M., 2007, ApJ, 660, 1556
	\bibitem[Rodriguez and Zuckerman 2012]{rodriguez12} Rodriguez, R., Zuckerman B., 2012, ApJ, 745, 147
	\bibitem[Santos et al. 2010]{santos10} Santos, N. C., Gomes da Silva, J., Lovis, C., Melo, C., 2010, A\&A, 511, 54
	\bibitem[Schneider et al. 2006]{schneider06} Schneider, G., Silverstone, M. D., Hines, D. C., et al, ApJ, 650, 414
	\bibitem[Schroeder et al. 2009]{schroeder09} Schroeder C., Reiners A., Schmidt, J.H.M.M., 2009, A\&A, 493, 1099
	\bibitem[Weise et al. 2010]{weise10} Weise, Launhardt, R, and Setiawan, J, 2010, A\&A, 517, 88
	\bibitem[Wright et al. 2004]{wright04} Wright, J. T., Marcy, G. W., Butler, R. P., Vogt, S. S., 2004, ApJS, 152, 261
	\bibitem[Zechmeister et al. 2009]{zechmeister09} Zechmeister, M., and Kuerster, M., 2009, A\&A, 496, 577
	\bibitem[Zuckerman et al. 2001]{zuckerman01} Zuckerman B., Song I., Bessel M.S. and Webb R.A. , et al, 2001, ApJ, 562, 87
\end{thebibliography}


